A Qualitative Analysis Framework for mHealth Privacy Practices

Mobile Health (mHealth) applications have become a crucial part of health monitoring and management. However, the proliferation of these applications has also raised concerns over the privacy and security of Personally Identifiable Information and Protected Health Information. Addressing these concerns, this paper introduces a novel framework for the qualitative evaluation of privacy practices in mHealth apps, particularly focusing on the handling and transmission of sensitive user data. Our investigation encompasses an analysis of 152 leading mHealth apps on the Android platform, leveraging the proposed framework to provide a multifaceted view of their data processing activities. Despite stringent regulations like the General Data Protection Regulation in the European Union and the Health Insurance Portability and Accountability Act in the United States, our findings indicate persistent issues with negligence and misuse of sensitive user information. We uncover significant instances of health information leakage to third-party trackers and a widespread neglect of privacy-by-design and transparency principles. Our research underscores the critical need for stricter enforcement of data protection laws and sets a foundation for future efforts aimed at enhancing user privacy within the mHealth ecosystem.

==> content/8_appendices.tex <==
\clearpage
\appendices

\onecolumn

\section{Mapping of PHI Classification Schemes}

\begin{figure}[h]
  \centering
  \includegraphics[width=.64\textwidth]{figures/data_mapping.pdf}
  \caption{Mapping of specificity and privacy labels to observed PII/PHI types. Due to a lack of fine-grained Google Play Privacy Label Subcategories for \textit{Fitness Info} and \textit{Health Info}, three supplemental subcategories are added to accurately reflect the observed PHI categories.}
  \label{fig:hoststats}
\end{figure}

\clearpage

\section{Synthetic Persona}
\label{app:persona}

==> tables/app_categories.tex <==
\begin{table}
  \centering
  \caption{Mapping of observed feature categories to app archetypes defined by Dehling et al., deriving the expected specificity of personal and health information available to the respective apps from the archetype.}
  \label{tab:appcategories}
  \begin{tabular}{lcccc}
    \toprule
    Feature Category & Apps & Archetype & PHI Specificity \\
    \midrule
    Screen Overlay    & 3   & AT 1      & Standard        \\
    Health Education  & 14  & AT 2      & Standard        \\
    Step Counter      & 4   & AT 5      & Nonstandard     \\
    Workout Tracker   & 26  & AT 5      & Nonstandard     \\
    Cardio Tracker    & 14  & AT 5      & Nonstandard     \\
    Diet Tracker      & 12  & AT 5      & Nonstandard     \\
    Wearable          & 3   & AT 5      & Nonstandard     \\
    Mental Wellbeing  & 6   & AT 5      & Nonstandard     \\
    Pharmacy          & 5   & AT 6      & Medical         \\
    Physician Finder  & 1   & AT 7      & Medical         \\
    Female Health     & 26  & AT 9      & Medical         \\
    Diagnostic        & 1   & AT 10     & Medical         \\
    Health Monitor    & 34  & AT 10     & Medical         \\
    Telemedicine      & 3   & AT 12     & Medical         \\
    \midrule
    Total             & 152 &           &                 \\
    \bottomrule
  \end{tabular}
\end{table}
